KEA: Tuning an Exabyte-Scale Data Infrastructure

Microsoft's internal big-data infrastructure is one of the largest in the world -- with over 300k machines running billions of tasks from over 0.6M daily jobs. Operating this infrastructure is a costly and complex endeavor, and efficiency is paramount. In fact, for over 15 years, a dedicated engineering team has tuned almost every aspect of this infrastructure, achieving state-of-the-art efficiency (>60% average CPU utilization across all clusters). Despite rich telemetry and strong expertise, faced with evolving hardware/software/workloads this manual tuning approach had reached its limit -- we had plateaued. In this paper, we present KEA, a multi-year effort to automate our tuning processes to be fully data/model-driven. KEA leverages a mix of domain knowledge and principled data science to capture the essence of our cluster dynamic behavior in a set of machine learning (ML) models based on collected system data. These models power automated optimization procedures for parameter tuning, and inform our leadership in critical decisions around engineering and capacity management (such as hardware and data center design, software investments, etc.). We combine "observational" tuning (i.e., using models to predict system behavior without direct experimentation) with judicious use of "flighting" (i.e., conservative testing in production). This allows us to support a broad range of applications that we discuss in this paper. KEA continuously tunes our cluster configurations and is on track to save Microsoft tens of millions of dollars per year. At the best of our knowledge, this paper is the first to discuss research challenges and practical learnings that emerge when tuning an exabyte-scale data infrastructure.

==> Background_old.tex <==
\section{Problem Description}\label{sec:background}

Yet-Another-Resource-Negotiator (YARN)~\cite{vavilapalli2013apache} is used in the analyzed cloud platform for the resource management and job scheduling (see Figure~\ref{fig:yarn}). 
\begin{figure}[H]
	\centering
	\includegraphics[width=\linewidth]{YARN.pdf}
	\caption{YARN}\label{fig:yarn}
	\Description{Components of YARN.}
\end{figure}
A resource manager manages the use of resources across the entire cluster; node managers (running on all the worker nodes) launch and monitor containers; application managers is in charge of the life-time monitoring of an application launched per job request. Each customer job consists of a large number of sub-tasks, or vertices, running across multiple nodes. And each vertex is executed by a container composed of a constrained set of resources (memory, CPU, and so on) on a node. The resource manager and node manager communicate in heartbeat messages to update their status on resource utilization. 

There are over hundreds of parameters in the YARN configuration file in the production system that might affect the system performance significantly.
Many of them are currently tuned by the engineers over the years based on their experiences of operating the system. Though, the majority are set to default. 
In this paper, we target the parameter of \verb|max_num_running_containers| that can be specified for different groups of machines. This number constrains the maximum number of containers that can be executed simultaneously on a node, and it is critical especially when the system is running with heavy workloads. Tuning this parameter for different machines shifts the workload significantly and affects the resource utilization accordingly. Similar approach can be used for tuning other parameters, such as \verb|max_queuing_length|, which will be discussed in more details in Section~\ref{sec:eval}. 


There are around 10-20 different machine stock keeping units (SKUs) in the cluster. They are in different geographic locations and with significant difference in hardware configurations. 
Figure~\ref{fig:count0} shows the number of machines in all the clusters with different SKUs and machine functions. There are two types of machine functions that correspond to working nodes in the cluster---"\verb|E2| " and "\verb|E3|". The others are related to the Resource Manager, the Autopilot system~\cite{isard2007autopilot}, etc.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.35\textwidth]{result//all_machine_count0}
	\caption{Machine count for different machine function and SKUs}\label{fig:count0}
\end{figure}

Among those machines, we noticed that the current workload assignment is not desirable. In general, we hope that faster machines can process more jobs and be better utilized. However, in most of the clusters, the slower machines with older SKUs, have higher CPU utilization levels (see Figure~\ref{fig:cpu} for instance). Therefore, we want to better tune the configuration to achieve better workload balance and improve efficiency.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.38\textwidth]{result//cpu_all}
	\caption{CPU Utilization level for all machine function and SKUs}\label{fig:cpu}
\end{figure}

With such heterogeneity, the max running containers should be set to different values for different SKU and machine functions to achieve the optimal performance. While the workload in different cluster also has significantly different characteristics (some are CPU heavy and some are memory heavy, etc.), the same configuration won't work for all the clusters. Therefore, the YARN configurations should be trained and tailored to each cluster with its workload based on different data inputs. 




==> Data.tex <==
\section{Performance Monitor}
\label{sec:data}

\KK{You probably don't need subsections in this section. You already talk about Vis. Service in the first subsection, so there is kind of duplicate text and we can gain space by dropping the subsections (and their titles that take space).}

\KK{I think there is a rule that figures should go in the top of columns (unless you can really not do otherwise). You can achieve this by doing the "t!" instead of "h" after the figure command.}

\KK{Check if we can mention the name of Aether.}

\KK{Instead of vertex ended, maybe you can mention "job events" or "job data" as a more generic way of mentioning that dataset. So you have job data, machine (runtime) data, and machine info.}

\KK{For the figure and the accompanying text: I am not sure if we care in the figure if it is Scope or Python scripts (you might (not 100\% sure) mention it in the text, but not in the figure for sure). Make simpler titles by mentioning the function of the rectangle instead, like "Feature Building", "Data Processing" (BTW too generic?), "Auto-tuning". What is PR? Is it pull request here? I would like to without searching the text. What is Cosmos repo? If auto-tuning produces a result, which I guess is new configurations, maybe add it in the arrow going to the PR.}

\KK{I think you can use the three "screenshots" of the visualization service to also convey a message, otherwise it is just some visualization that is taking up space without being too important. For example, you can use some of these figures in the Background Section (Section 2) if you want to say some evidence data about our clusters and then you can refer to those figures again here to say "BTW this is done by our visualization service". Of course let's do that only if it makes sense in that section. But I'd expect we can use these figures for more than "this is what our users can see in our visualization".}

\subsection{Data Orchestration}
To support the various KEA applications, we first developed the data pipeline to automatically collect the telemetry data on a daily basis. We use Aether to host the end-to-end data collection pipeline and manage the computation jobs, which is a stable internal service to perform data processing tasks, similar to the Azure Machine Learning~\cite{aml}, and it has been used by multiple teams within the company.
In this section, we discuss the two main components for the performance monitor: i) the Aether pipeline and ii) the visualization service (see Figure~\ref{fig:architecture2}).

The \textbf{Aether Pipeline} is used to submit Scope scripts~\cite{chaiken2008scope} to collect data from Cosmos, execute Python scripts for pre-processing or running the machine learning algorithms/optimization to obtain new configuration suggestions. Aether is able to access the data from the Cosmos storage and submit Scope query jobs (see Figure~\ref{fig:architecture2}). The data sources consist of: (i) information at the job and vertex level from the \textit{Vertex Ended} event logs, (ii) the heartbeat of each machine indicating the CPU utilization level, number of containers running by time of day, etc. from the \textit{Machine Counter} dataset, and (iii) information on each machine configuration in the cluster from the \textit{Machine Info} dataset. The Python modules access the output data from Cosmos jobs, combine the data sources by timestamps and machine names and save the processed data to Cosmos for other usage. For some of the applications, the tuning modules can also be hosted on Aether. In this case, the processed data will be fed to downstream modules such as the auto-tuning module to propose new configurations to the cluster. A Pull Request (PR) can be created automatically to deploy the new configuration file to the Cosmos repository.

The \textbf{Visualization Service}, currently called Cosmoslook, is hosted as a Bokeh service~\cite{bokeh} on a corporation machine within the company Ethernet. It consumes the data from Cosmos and hosts the visualization dashboard. %
The machine downloads the processed data using a pre-installed certificate for authentication, protected by a password. 
The visualization dashboard (with aggregated statistics) is hosted on a port of this machine and it can be accessed within the company Ethernet. 



\subsection{Visualization Service}
The visualization service provides multiple views and user interaction widgets such as a drop-down menu to choose the cluster, SKU, performance counter, etc. to visualize.
\KK{Nit: in various places, when you mention "such" by definition it is non-inclusive, so no need for "etc.".}

The scatter view shows the data at the dis-aggregate level (see Figure~\ref{fig:scatter2}). Users can choose to visualize the daily/hourly data and different machine functions/SKUs. Each point corresponds to one observation, i.e. one machine for one hour or one day. A hover tool is provided to show the machine name, machine function and SKU for the selected data points for quick debugging of engineers. Users can choose from more than 60 counters to visualize as the x/y-axis. A slider was provided to select the time range of the data.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\textwidth]{cosmoslook//Scatter_edit}
	\caption{Scatter View of Cosmoslook}\label{fig:scatter2}
\end{figure}

The Empirical Cumulative Distribution Function (ECDF) view shows the distribution of the performance counters. The visualization can be grouped by machine functions, SKUs, or the combination of the two. It provides a good comparison between different groups of machines about their performance.

The boxplot view shows the distribution of data points by different time of day/week. Similarly, users can choose from the daily view or the hourly view and visualize different performance metrics (see Figure~\ref{fig:box2}).

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\textwidth]{cosmoslook//Boxplot}
	\caption{Boxplot View of Cosmoslook}\label{fig:box2}
\end{figure}

Based on different applications, more views are being added according to the analytic needs, such as the token usage for different customers by time of day.




==> E2E3.tex <==
\section{Selecting Best Machine Functions}\label{sec:e2e3}

In this section, we discuss the KEA application on selecting the best machine functions between ``E2" and ``E3". For this application, we start with the flighting module to test out the performance of the machines with different machine functions.

\subsection{Flighting}
Similar to the experiments for power capping, we select a podset of 700 machines and update the machine function for every other machine from E2 to E3. Therefore, we have 350 machines with E2 and 350 with E3. In this case, we also make sure that the two groups of machines are receiving very similar workloads throughout the experiment. For all the experiments, we collected data for the two groups of machines with the same SKU for both the time period before the conversion and after.

In each round of the flighting, we selected 120 machines for each group and capped the machines at 10\%, 15\%, 20\%, 25\% and 30\% below the original power provision level respectively and kept running for more than 24 hours.

\subsection{Modeling}

For all the sampled data, other than the power consumption level and the throttling counts, we also collect Bytes\_per\_CPU\_Time (defined as the TotalDataRead/Total CPU Time for all vertices on each machine) and Bytes\_per\_Second (defined as the TotalDataRead/Total Vertex Execution Time) as the main performance metrics. The two metrics are proved to be less sensitive to workload levels compared to the others, such as latency measurements. Student t-test was conducted to evaluate the significance of the performance change. 

Fig.~\ref{fig:pc} shows the performance impact on the two metrics due to different power capping levels for Gen 4 machines (includes all the SKUs with ending with ``15") with/without Turbo enabled. The y-axis indicates the performance change bench-marked to the baseline, i.e. Group A with no capping and Turbo off. We can see that with the increasing power capping level, the impact of capping becomes more significant. And in all cases, with Turbo turning-on improves on the performance.

\begin{figure}[h]
	\centering
	\begin{minipage}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{powercapping/pc}
	\end{minipage}%
	\caption{Performance impact due to power capping}\label{fig:pc}
\end{figure}

Similar experiments are also conducted for other SKUs in different clusters to determine the best level of power provision. Eventually, a relatively conservative capping level is chosen, though still much lower than the origin level, which leads to around 80 GWh lower power consumption per year and large cost-saving in the scale of tens of million dollars.




==> MachineFunction.tex <==
\subsection{Selecting Best Machine Functions}\label{sec:e2e3}

\KK{Here I have similar questions as in the power capping section.}

In this section, we discuss the KEA application on selecting the best machine functions between \verb|E2| and \verb|E3|. The \verb|E2| predates the \verb|E3|, and the creation of the \verb|E3| design was motivated by high D drive write latency on \verb|E2|s caused by contention for I/O on the HDD. Specifically, the YARN resource localization for containers is done on D drive in Cosmos, and in the \verb|E2| configuration, we experienced extremely high resource localization latency. This latency was in the hot path for launching Scope vertices and directly impacted the performance of Cosmos jobs. We moved the D drive to SSD for \verb|E3| machines because an SSD can support more Input/Output Operations Per Second (IOPS) at lower latency. This configuration change aims at resolving the resource localization bottleneck in our system. 

At the time that the \verb|E3| configuration was validated in production we decided that all new servers added to our system would be configured as \verb|E3| rather than \verb|E2|. For the thousands of existing \verb|E2| in production we decided to leave them as \verb|E2|s to avoid the significant effort required to convert them. The process of converting an existing machine from \verb|E2| to \verb|E3| is slow because we have to move the data off the machines to reconfigure them. We had tens of thousands of \verb|E2| machines in our clusters that would need to be manually converted in very small batches and we did not think this reconfiguration was worth the effort. 

However, this analysis from KEA later showed the significance of the performance improvement from using \verb|E3|, which motivated us to spend months converting all servers that had sufficient SSD capacity from the \verb|E2| to the \verb|E3| configuration. The only servers which were not converted to \verb|E3| were the V14 machines which did not have enough SSD to support the D drive.

\subsection{Flighting}
Similar to the experiments for power capping, we select a group of 700 machines and update the machine function for every other machine from \verb|E2| to \verb|E3|. Thus, we have 350 machines with \verb|E2| and 350 with \verb|E3|. This setting ensures that the two groups of machines are receiving almost identical workloads throughout the experiment. For all the experiments, we collected data for the two groups of machines with the same SKU for both the time periods before the conversion and after.

\subsection{Modeling}

Table.~\ref{table:e2e3} shows the performance impact due to the change of machine functions for the two groups of machines with 5-day's observation. 
The Total Data Read per day increased by 10.9\% while the average vertex latency decreased by 5.2\%, which is very significant improvement. And the result for Student's t-test shows that the changes are all significant.

\begin{table}[h]
		\caption{Performance metrics for E2 and E2 machiens}\label{table:e2e3}
	\begin{tabular}{lllcl}
		    		\toprule
		Name                     & \verb|E2|      & \verb|E3|      & \% Changes & t-value\\ \midrule
		Total Data Read (PB)    &1.38   & 1.53 & 10.9\%  & 40.4   \\
		Average Vertex Executiontime       &24.1   & 22.9 & -5.2\%  &27.1   \\
		Total CPU Time ($\cdot 10^{12}$)               & 0.32 & 0.36 & 12.3\% &74.2    \\
		Bytes per CPU time    & 4.29   & 4.31     & 0.3\%  &1.65    \\
		Average Running Containers &  7.67   & 8.00    & 4.3\%  &38.2    \\
		Norm Execution Time ($\cdot 10^{-5}$)      &  1.71 &1.82 & -5.8\%  &32.8   \\ \bottomrule
	\end{tabular}
\end{table}




==> OverSubscribe.tex <==
\subsection{Oversubscribing Clusters}\label{sec:oversub}

In this section, we discuss the KEA application on determining the optimal over-subscription ratio to improve the system utilization and designing the new pricing regime.

In this analyzed system, there has been a lot of discussion to improve on the utilization of the current capacity, and various engineering efforts have been made to better utilize the idle capacity~\cite{curino2019hydra}. One proposal is to overbook the cluster capacity by over-selling the tokens.

A new offer of cheaper ``Perf Tokens" is proposed for the off-peak period to attract customers to schedule their jobs during this time period thus reduce the workload pressure during the peak periods. Based on historic demand patterns, we can better design this offer to help customers reduce cost, guide them to use the idle capacity with cheaper prices, and further improve the resource utilization of the current capacity. This project is a joint effort with the PM team and the engineering team. The research results provide a good evaluation for the different design of the pricing regime and examine the corresponding financial impacts. 


The key challenge is to estimate the new demand pattern given (i) over-subscription and (ii) the Perf Token offer. Thus, in the What-if Engine, we want to estimate the resulting demand profile, and the total revenue of the cluster given different pricing offers to customers and over-subscription ratios. And in the Optimizer, we pick the optimal solution.

KEA data pipeline records the detailed cluster utilization level since its deployment for all the production clusters. We used the current utilization pattern to infer the future demand with over-subscription and the Perf Token offer as two separate steps. 
First, we estimate the new demand usage based on the over-subscription ratio. And second, we estimate the peak spreading with the cheaper Perf Token offers during the off-peak. We evaluate the financial impact with 1600 scenarios in the What-if Engine, e.g. with different levels of Perf Token discount, different over-subscription ratios, etc., by incorporating the financial costs and perform the optimization.


Figure~\ref{fig:base} shows the current utilization for the cluster for two types of customer demand (guaranteed high priority tokens and low priority tokens) for one of clusters with around 37,000 machines. The blue line shows the usage for the high priority tokens and the orange for all the tokens. The y-axis shows the number of total number of containers running in the cluster by time of day. We can see that there is clearly a repetitive pattern in the cluster, and the usage in the early morning is usually high. 

\begin{figure}[!t]
	\centering
	\begin{minipage}[b]{0.5\textwidth}
		\includegraphics[width=\textwidth]{oversubscription/short_term_cosmos09.pdf}
	\end{minipage}%
	\caption{Current usage for one of the cluster}\label{fig:base}
\end{figure}

\subsubsection*{\textbf{Over-Subscription}}
The idea of over-subscription is to increase the total demand even to the extent that, for a short period of time, the demand might exceed the current capacity (i.e. the green line in Figure~\ref{fig:base}). The extra demand will be incorporated by ad-hoc purchased Azure capacity, which is more costly compared to the existing capacity. However, we also increase the utilization during the off-peak, thus reduce the total cost per container. In this research, we are looking for the optimal level of over-subscription thus the cost reduction is maximized. We assume that the base demand will increase in proportional to the over-subscription ratio bench-marked to the current observations. In this sense, the un-changed aspect of the system is the baseline demand pattern.

\subsubsection*{\textbf{Perf Token Offer}} The idea of Perf Token is to encourage customers to shift from the peak period to the off-peak, which is a common practice in many other industries~\cite{elmaghraby2003dynamic}, such as the congestion pricing in transportation~\cite{de2011traffic,lindsney2001traffic}, time of use billing in utility supply~\cite{torriti2012price}, spot-pricing in cloud computing~\cite{agmon2013deconstructing}, etc. For Perf Token offers, we hope to leverage the idle capacity during the off-peak and offer them to customers with a lower price thus, to some extent, reduce the peak load and increase it for the off-peak. 


Figure~\ref{fig:typical} shows the number of containers running for each hour of day based on historic observation over 4-month's data and the corresponding different percentiles. The total amount of Perf Tokens that can be offered is determined by its duration and how aggressively we want to offer them to customers with different levels of availability guarantees based on the remaining idle capacity. We define a \textit{Perf Token period} that restricts the time period that the Perf Tokens can be used. This is very similar to fit a rectangle into Figure~\ref{fig:typical}. 

\begin{figure}[!t]
	\centering
	\begin{minipage}[b]{0.5\textwidth}
		\includegraphics[width=\textwidth]{oversubscription/typical_day_cosmos09.pdf}
	\end{minipage}%
	\caption{A typical day of demand request}\label{fig:typical}
\end{figure}

Figure~\ref{fig:perftoken} shows the availability of the Perf Token given different levels of availability probabilities and duration. Based on the current observed demand, we can offer 120,008 Perf Tokens if we ensure that the probability of this amount of tokens to be available for 4 hours is larger than 75\% (see left in Figure~\ref{fig:perftoken}). Similarly, with a higher level of promise, this number will decrease as we want to offer the Perf Tokens more conservatively. On the other hand, with longer Perf Token period, the amount of available Perf Tokens also decreases (see right in Figure~\ref{fig:perftoken}). Therefore, the duration and Service Level Agreement (SLA) levels are important inputs/decision variables for this model that we will enumerate upon in different scenarios.

\begin{figure}[!t]
	\centering
	\begin{minipage}[b]{0.25\textwidth}
		\includegraphics[width=\textwidth]{oversubscription/perf_token_4_duration.pdf}
	\end{minipage}%
		\begin{minipage}[b]{0.25\textwidth}
			\includegraphics[width=\textwidth]{oversubscription/perf_token_8_duration.pdf}
		\end{minipage}%
	\caption{A typical day of demand request}\label{fig:perftoken}
\end{figure}

Because of the Perf Token offers, customers will enjoy a cheaper price of scheduling jobs during the pre-defined off-peak period. In this sense, we would expect the demand profile to change. Specifically, some of the demand during the peak period will shift to the off-peak period. Moreover, we can expect that more demand will shift around the boundary between the peak and off-peak periods. 

Consumer behavior with respect to different pricing regime has been well studied in previous literature. 
Focusing on behavior aspects, choice models have been widely used to estimate the consumer choices at the individual level~\cite{mcfadden1974measurement, luce2012individual, rao1993pricing,mcfadden1980econometric}. A utility function was constructed to represent the attractiveness of each product or alternative for each customer. Their perception about the brand price, quality of goods, and brand values can be included~ 
\cite{lichtenstein1989relationship,zeithaml1988consumer,curry1988prices,rao1989effect}. 
\cite{akccay2010joint} introduced a linear function to capture the utility of purchasing a product as a function of its value and price for a customer.  
~\cite{broder2012dynamic} developed a forced-exploration policy to search for the optimal pricing policy to maximize revenue. The parameters for the choice model were estimated assuming different forms of parametric demand curves, such as logit demand (in the class of discrete choice model), linear demand and exponential demand as a function of price. \cite{yan2019dynamic} used logit model to estimate the demand response with respect to dynamic pricing using data from a ride-hailing platform. They modeled the utility of passengers as a function of price, wait time and time of day. 

In this paper, we introduce the similar demand modeling method, the logit model to estimate the potential shift of demand during different times of day due to the Perf Token offer. And this demand modeling is another key element for the un-changed system characteristics that we leverage to make prediction for un-existing scenarios. 

This model captures:
\begin{enumerate}
	\item The \textbf{inertia of shifting jobs}. With the same token cost, customers will prefer their original job scheduling time. They are less likely to change job scheduling dramatically but try to shift as little as possible to benefit from the cheaper tokens.
	\item The \textbf{price} of using different tokens. The cheaper the price is the more likely it is to attract more usage.
\end{enumerate}

In this model, we assume that each customer is making a choice between scheduling the job at the original time versus some other times. We define the utility function as below for a customer to use a token in hour $X (X=0,1,2\cdots23)$ while the preferred time is $X_0$, which is the original time the job is scheduled from the current observed demand:
\begin{equation} \label{eq:logit2}
U(X)= \alpha|X-X_0 |+ \beta D(X),
\end{equation}
where $D(X)$ is the token price at time $X$. 
$\alpha$ and $\beta$ are parameters representing the sensitivity of customers to time shifting and price. 
A customer will choose to use a token at time $X$ with probability:
\begin{equation} \label{eq:logit}
P(X)=  \frac{\exp^{U(X)}}{\sum_{x'=0}^{23} \exp^{U(x')}}.
\end{equation}
If a customer is extremely time sensitive, i.e. $\alpha=-\inf$, we will have $P(X_0)=1$ and $P(X)=0$ $\forall X\neq X_0$. On the other end, if the customer is extremely price sensitive, i.e. $\beta=-\inf$, we will have $P(X)=0$ for $X$ not in the Perf Token period.
The parameters of time sensitivity $\alpha$ and price sensitivity $\beta$ can be estimated using Maximum Likelihood Estimation (MLE)~\cite{train2009discrete} by the realized demand or conducting surveys on customer's willingness to take different offers, e.g. giving $p$ \% discount for Perf Tokens, if they are willing to shift jobs for $\Delta X$ hours. In this research, sensitivity analysis was conducted to evaluate the results with respect to different values of $\alpha$ and $\beta$.

For each token's usage for each hour, we redistribute the demand based on equation~\eqref{eq:logit}. Figure~\ref{fig:discount} shows the estimated demand shift due to the Perf Tokens given different discount levels assuming no capacity limit. The green line shows the demand that has the time flexibility to shift in the analyzed cluster. With higher levels of price discount for the Perf Token (the orange line), more demand will shift to the Perf Token period. We can also see that the demand increases the most right after the starting of the Perf Token period. This is inevitable as customers are in general reluctant to shift jobs and they want to change their schedule as little as possible and still take advantage of the cheaper tokens.

\begin{figure}[!t]
	\centering
	\begin{minipage}[b]{0.5\textwidth}
		\includegraphics[width=\textwidth]{oversubscription/sensitivity222.pdf}
	\end{minipage}%
	\caption{Demand shift with different discount levels}\label{fig:discount}
\end{figure}

As discussed in the previous section, we only have a limited number of Perf Tokens available given different levels of availability promises/SLAs. Therefore, we implement a constrained logit model to re-estimate the demand shifting behavior with limited Perf Token capacity~\cite{de2007discrete}. Figure~\ref{fig:shift} shows the new demand curve with the Perf Token offer with 75\% SLA level and 30\% discount offered during 16:00-00:00. We can see that the demand curve is effectively ``flattened". We also make the crucial observation that the demand for Perf Tokens in general exceeds the availability, therefore, the estimation is more sensitive to the availability of Perf Tokens instead of the price and time sensitivity parameters as in equation~\eqref{eq:logit2}.

\begin{figure}[!t]
	\centering
	\begin{minipage}[b]{0.5\textwidth}
		\includegraphics[width=\textwidth]{oversubscription/short_term_cosmos09_shifted_constraint_total.pdf}
	\end{minipage}%
	\caption{Demand shift with different discount levels}\label{fig:shift}
\end{figure}

As the peak demand is reduced, we can further over-subscribe the cluster to a higher level thus increase the total utilization level and reduce the cost. Incorporating the real cost figures, the optimal over-subscription ratio for most of the clusters is 20\%. Based on different design of Perf Token offers, for the 5 biggest production clusters, in the optimal cases, i.e. with the optimal levels of over-subscription and pricing, we can reduce on average 6\% of the cost per container scheduled for customers, which corresponds to tens of million dollars saving per year. 


For the analyzed system, this type of incentive is relatively new to customers. A pilot experiment on this offer will be conducted with a selected group of customers and more data will be available to validate this analysis and fine-tune the models. 

